Benchmarking Generative AI Models for Deep Learning Test Input Generation

Test Input Generators (TIGs) are crucial to assess the ability of Deep Learning (DL) image classifiers to provide correct predictions for inputs beyond their training and test sets. Recent advancements in Generative AI (GenAI) models have made them a powerful tool for creating and manipulating synthetic images, although these advancements also imply increased complexity and resource demands for training. In this work, we benchmark and combine different GenAI models with TIGs, assessing their effectiveness, efficiency, and quality of the generated test images, in terms of domain validity and label preservation. We conduct an empirical study involving three different GenAI architectures (VAEs, GANs, Diffusion Models), five classification tasks of increasing complexity, and 364 human evaluations. Our results show that simpler architectures, such as VAEs, are sufficient for less complex datasets like MNIST. However, when dealing with feature-rich datasets, such as ImageNet, more sophisticated architectures like Diffusion Models achieve superior performance by generating a higher number of valid, misclassification-inducing inputs.

==> table-for-trainingtime-infertime.tex <==
\begin{table}[t]
\caption{Training and Inference Times of Generative Models}
\label{tab:training_inference_times}
\centering
\begin{tabular}{|p{1.5cm}|p{2.0cm}|p{3.0cm}|p{2.0cm}|}
\hline
\textbf{Dataset} & \textbf{Model} & \textbf{Training-Time(min,sec)} & \textbf{Inference-Time(ms)} \\ \hline
\textbf{MNIST} & VAE & 6 min 12.33 sec & 0.27 \\ 
 & GAN & 120 min 45 sec & 0.7 \\ 
 & SD & 404 min 45.6 sec & 960.68 \\ \hline
\textbf{SVHN} & VAE & 93 min 29.74 sec & 4.07 \\ 
 & GAN & 86 min 28.83 sec & 1.75 \\ 
 & SD & 572 min 24 sec & 1213.49 \\ \hline
\textbf{CIFAR10} & VAE & 423 min 36 sec & 2.51 \\ 
 & GAN & 450 min 0 sec & 1.73 \\ 
 & SD & 362 min 24 sec & 1903.29 \\ \hline
\textbf{Imagenet} & VAE & 2520 min 36 sec & 11.92 \\ 
 & GAN & 21600 min 0 sec & 20.68 \\ 
 & SD & 30 min 1.8 sec & 1945.77 \\ \hline
\end{tabular}
\end{table}


